Depth as Time in One-Step Generative Models

The recent wave of one-step generative models, which compress the multi-step trajectory of diffusion via either distillation or learned flow maps, has reached an inflection point where they can generate high-quality images. Here, we ask a natural question that follows from these advances: what happens to the denoising trajectory of multi-step diffusion when generation is compressed into a single forward pass? We offer an empirical observation we call \textit{depth as time}: the denoising computation that multi-step diffusion performs across sampling steps appears to unfold across the depth of a single forward pass, and can be recovered by decoding intermediate layers with the model's own output head. Most interestingly, we show that this depthwise computation depends on the transport task a flow map is trained to solve. The most surprising case is MeanFlow, where probing shorter transport intervals reveals both denoising and renoising within a single network evaluation. In contrast, generators trained without a time-indexed transport task, such as drifting models, do not exhibit the same depthwise denoising. Consequently, we show that models that exhibit the depthwise denoising phenomenon are more compressible across the layerwise computation: a MeanFlow \texttt{SiT-L/2} model can be compressed by $16.6\times$ in parameters into a single time-conditioned block. We offer an explanation for this denoise-then-renoise behavior and show that, when we treat the layerwise computation explicitly as a flow, a single time-conditioned block can be trained to denoise across layers, compressing a MeanFlow \texttt{SiT-L/2} model by $16.6\times$ in parameters. Together, these results suggest that the temporal computation of diffusion is not eliminated by one-step generation, but reorganized across network depth.

==> tables/imagenet-256.tex <==
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1pt}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1pt}}

\begin{table*}[!ht]
\centering
\scriptsize

\begin{minipage}{0.7\textwidth}
\centering
\setlength{\tabcolsep}{4pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{L{111}x{30}x{150}R{12}R{10}R{10}}

method & space & params $\downarrow$  & NFE & FID $\downarrow$ & IS $\uparrow$ \\

\specialrule{\lightrulewidth}{\aboverulesep}{0.5pt}
\rowcolor{gray!15}
\multicolumn{6}{l}{%
  \textit{Multi-step Diffusion/Flows}%
} \\
~~\textcolor[HTML]{808080}{DiT-XL/2~\citep{peebles2023scalable}}
  & \textcolor[HTML]{808080}{{\scriptsize SD-VAE}}
  & \textcolor[HTML]{808080}{675M}
  & {\scriptsize \textcolor[HTML]{808080}{250 $\times$ 2}}
  & \textcolor[HTML]{808080}{2.27}
  & \textcolor[HTML]{808080}{278.2}\\

~~\textcolor[HTML]{808080}{SiT-XL/2~\citep{ma2024sit}}
  & \textcolor[HTML]{808080}{{\scriptsize SD-VAE}}
  & \textcolor[HTML]{808080}{675M}
  & {\scriptsize \textcolor[HTML]{808080}{250 $\times$ 2}}
  & \textcolor[HTML]{808080}{2.06}
  & \textcolor[HTML]{808080}{277.5}\\

~~\textcolor[HTML]{808080}{SiT-XL/2+REPA~\citep{yu2024representation}}
  & \textcolor[HTML]{808080}{{\scriptsize SD-VAE}}
  & \textcolor[HTML]{808080}{675M}
  & {\scriptsize \textcolor[HTML]{808080}{250 $\times$ 2}}
  & \textcolor[HTML]{808080}{1.42}
  & \textcolor[HTML]{808080}{305.7}\\

~~\textcolor[HTML]{808080}{LightningDiT-XL/2~\citep{11094598}}
  & \textcolor[HTML]{808080}{{\scriptsize SD-VAE}}
  & \textcolor[HTML]{808080}{675M}
  & {\scriptsize \textcolor[HTML]{808080}{250 $\times$ 2}}
  & \textcolor[HTML]{808080}{1.35}
  & \textcolor[HTML]{808080}{295.3} \\

~~\textcolor[HTML]{808080}{RAE-DiT$^\text{DH}$-XL/2~\citep{zheng2026diffusion}}
  & \textcolor[HTML]{808080}{{\scriptsize RAE}}
  & \textcolor[HTML]{808080}{839M}
  & {\scriptsize \textcolor[HTML]{808080}{50 $\times$ 2}}
  & \textcolor[HTML]{808080}{1.13}
  & \textcolor[HTML]{808080}{262.6}\\

\specialrule{\lightrulewidth}{\aboverulesep}{0.5pt}
\rowcolor{gray!15}
\multicolumn{6}{l}{%
  \textit{One-step latent-space generation}%
} \\

~~iCT-XL/2~\citep{song2023improved}
  & {\scriptsize SD-VAE}
  & 675M
  & {\scriptsize 1}
  & {\scriptsize 34.24}
  & - \\

~~Shortcut-XL/2~\citep{frans2024one}
  & {\scriptsize SD-VAE}
  & 675M
  & {\scriptsize 1}
  & {\scriptsize 10.60}
  & - \\

~~MeanFlow-L/2~\citep{geng2025mean}
  & {\scriptsize SD-VAE}
  & 459M
  & {\scriptsize 1}
  & {\scriptsize 3.84}
  & - \\

~~MeanFlow-B/2~\citep{geng2025mean}
  & {\scriptsize SD-VAE}
  & 131M
  & {\scriptsize 1}
  & {\scriptsize 6.17}
  & - \\

\specialrule{\lightrulewidth}{\aboverulesep}{2pt}

~~\textbf{Depth-as-Time-B/2}\,
\textcolor[HTML]{1E4E8C}{\scalebox{0.9}{\texttt{nub=1}}}
  & {\scriptsize SD-VAE}
  & \cellcolor[HTML]{EAF2FB}%
    \makebox[5.5em][l]{%
      {\scriptsize 16M}\,
      \scalebox{0.75}{%
        \textcolor[HTML]{1E4E8C}{\((8.2\times)\)}
      }
    }
  & {\scriptsize $1{\times}2$}
  & {\scriptsize 8.17}
  & \\

~~\textbf{Depth-as-Time-B/2}\,
\textcolor[HTML]{1E4E8C}{\scalebox{0.9}{\texttt{nub=2}}}
  & {\scriptsize SD-VAE}
  & \cellcolor[HTML]{EAF2FB}%
    \makebox[5.5em][l]{%
      {\scriptsize 27M}\,
      \scalebox{0.75}{%
        \textcolor[HTML]{1E4E8C}{\((4.9\times)\)}
      }
    }
  & {\scriptsize $1{\times}2$}
  & {\scriptsize 5.84}
  & \\

~~\textbf{Depth-as-Time-L/2}\,
\textcolor[HTML]{1E4E8C}{\scalebox{0.9}{\texttt{nub=1}}}
  & {\scriptsize SD-VAE}
  & \cellcolor[HTML]{EAF2FB}%
    \makebox[5.5em][l]{%
      {\scriptsize 28M}\,
      \scalebox{0.75}{%
        \textcolor[HTML]{1E4E8C}{\((16.7\times)\)}
      }
    }
  & {\scriptsize $1{\times}2$}
  & {\scriptsize 4.87}
  & \\

~~\textbf{Depth-as-Time-L/2}\,
\textcolor[HTML]{1E4E8C}{\scalebox{0.9}{\texttt{nub=2}}}
  & {\scriptsize SD-VAE}
  & \cellcolor[HTML]{EAF2FB}%
    \makebox[5.5em][l]{%
      {\scriptsize 47M}\,
      \scalebox{0.75}{%
        \textcolor[HTML]{1E4E8C}{\((9.9\times)\)}
      }
    }
  & {\scriptsize $1{\times}2$}
  & {\scriptsize 4.04}
  & \\

\specialrule{\lightrulewidth}{\aboverulesep}{0.5pt}
\rowcolor{gray!15}
\multicolumn{6}{l}{%
  \textit{One-step pixel-space generation}%
} \\

~~PixelDiT/16~\citep{yu2026pixeldit}
  & {\scriptsize pixel}
  & 797M
  & {\scriptsize $200{\times}2$}
  & {\scriptsize 1.61}
  & 292.7 \\

~~JiT-G/16~\citep{li2026back}
  & {\scriptsize pixel}
  & 2B
  & {\scriptsize $100{\times}2$}
  & {\scriptsize 1.82}
  & 292.6\\

~~EPG-L/16~\citep{liu2026there}
  & {\scriptsize pixel}
  & 540M
  & {\scriptsize 1}
  & {\scriptsize 8.82}
  & - \\

~~pMF-L/16~\citep{lu2026one}
  & {\scriptsize pixel}
  & 410M
  & {\scriptsize 1}
  & {\scriptsize 2.52}
  & 262.6\\

\specialrule{\lightrulewidth}{\aboverulesep}{2pt}

~~\textbf{Depth-as-Time-L/16}\,
\textcolor[HTML]{1E4E8C}{\scalebox{0.9}{\texttt{nub=1}}}
  & {\scriptsize pixel}
  & \cellcolor[HTML]{EAF2FB}%
    \makebox[5.5em][l]{%
      {\scriptsize 34M}\,
      \scalebox{0.75}{%
        \textcolor[HTML]{1E4E8C}{\((19.5\times)\)}
      }
    }
  & $1{\times}2$
  & \textbf{--}
  & \\

~~\textbf{Depth-as-Time-L/16}\,
\textcolor[HTML]{1E4E8C}{\scalebox{0.9}{\texttt{nub=2}}}
  & {\scriptsize pixel}
  & \cellcolor[HTML]{EAF2FB}%
    \makebox[5.5em][l]{%
      {\scriptsize 58M}\,
      \scalebox{0.75}{%
        \textcolor[HTML]{1E4E8C}{\((11.5\times)\)}
      }
    }
  & $1{\times}2$
  & \textbf{--}
  & \\

\bottomrule
\end{tabular}%
}

\end{minipage}

\caption{%
  \textbf{Class-conditional generation on ImageNet-$256{\times}256$.}
  We compare Depth-as-Time with multi-step diffusion and flow models
  and one-step generative models operating in latent or pixel space.
  We report model parameters, number of function evaluations (NFE),
  FID-50k, and Inception Score (IS).
  All results use classifier-free guidance (CFG) when applicable;
  ``$\times 2$'' denotes the additional function evaluation required
  by CFG at each sampling step.
  For Depth-as-Time, the blue values in parentheses report parameter
  reduction relative to the corresponding teacher model.
  % $^{\dagger}$iCT~\citep{song2023improved} results are reported by~\citep{zhou2025inductive}.
}
\label{tab:all_results}

\vspace{-0.5em}
\end{table*}
